Efficient Long Video Tokenization via Coordinate-based Patch Reconstruction

Efficient tokenization of videos remains a challenge in training vision models that can process long videos. One promising direction is to develop a tokenizer that can encode long video clips, as it would enable the tokenizer to leverage the temporal coherence of videos better for tokenization. However, training existing tokenizers on long videos often incurs a huge training cost as they are trained to reconstruct all the frames at once. In this paper, we introduce CoordTok, a video tokenizer that learns a mapping from coordinate-based representations to the corresponding patches of input videos, inspired by recent advances in 3D generative models. In particular, CoordTok encodes a video into factorized triplane representations and reconstructs patches that correspond to randomly sampled $(x,y,t)$ coordinates. This allows for training large tokenizer models directly on long videos without requiring excessive training resources. Our experiments show that CoordTok can drastically reduce the number of tokens for encoding long video clips. For instance, CoordTok can encode a 128-frame video with 128$\times$128 resolution into 1280 tokens, while baselines need 6144 or 8192 tokens to achieve similar reconstruction quality. We further show that this efficient video tokenization enables memory-efficient training of a diffusion transformer that can generate 128 frames at once.

==> resource/analysis_scalability_table.tex <==
\begin{table*}[t]
\centering
\subfloat[
\textbf{Model size scalability.} xx
\label{table:model_size}
]{
\centering
\begin{minipage}{0.33\linewidth}
\begin{center}
\scriptsize
\tablestyle{3pt}{1.2}
\begin{tabular}{lcc}
\toprule \\
Model size & rFVD$\downarrow$ & PSNR$\uparrow$ \\
\midrule
Small & \\
Base & \\
Large &  \\
\bottomrule
\end{tabular}
\end{center}
\end{minipage}
}
\hspace{1em}
\subfloat[
\textbf{Token size scalability - Spatial.} xx
\label{table:token_size_spatial}
]{
\centering
\begin{minipage}{0.45\linewidth}
\begin{center}
\scriptsize
\tablestyle{3pt}{1.2}
\begin{tabular}{lccc}
\toprule \\
Token size & $xy$ plane shape & rFVD$\downarrow$ & PSNR$\uparrow$ \\
\midrule
Small & \\
Base & \\
Large &  \\
\bottomrule
\end{tabular}
\end{center}
\end{minipage}
}
\hspace{1em}
\subfloat[
\textbf{Token size scalability - Temporal.} xx
\label{table:effect_auxiliary_mae}
]{
\centering
\begin{minipage}{0.45\linewidth}
\begin{center}
\scriptsize
\tablestyle{3pt}{1.2}
\begin{tabular}{lccc}
\toprule \\
Token size & $yt$ and $xt$ plane shape &rFVD$\downarrow$ & PSNR$\uparrow$ \\
\midrule
Small & \\
Base & \\
Large &  \\
\bottomrule
\end{tabular}
\end{center}
\end{minipage}
\vspace{-0.025in}
\caption{\textbf{Scalability analysis on CoordTok.} We report the performance xx. (a) Model size: (Small, Base, Large), (b) Spatial: (\textbf{16$\times$16}, $32\times32, 64\times64$; Temporal 32 fixed), (c) Temporal: (16, \textbf{32}, 64; Spatial $16\times16$). Note that our reporting setup is spatial $16\times16$ and temporal 32}
\label{table:ablations1} 
\vspace{-0.15in}
\end{table*}

==> resource/generation_curve.tex <==
\begin{figure}[t]

\centering\small
    \includegraphics[width=0.9\linewidth]{assets/gen_fvd_curve.pdf}
    \vspace{-0.1in}
    \caption{Unconditional 128-frames, 128$\times$128 resolution video generation for our CoordTok with different token sizes, trained on UCF-101 dataset.}
    \label{fig:generation_fvd_curve}
\end{figure}

==> resource/qualitative_results_gen.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{assets/qualitative_results_gen_v2.pdf}
\vspace{-0.1in}
\caption{\textbf{Unconditional 128-frame, 128$\times$128 resolution video generation results} from CoordTok-SiT-L/2 trained on 128-frame videos from the UCF-101 dataset \citep{soomro2012ucf101}.
We provide more examples of generated videos in \cref{appendix:additional_qualitative_results}.}
\label{fig:qualitative_results_gen}
\vspace{-0.1in}
\end{figure*}

==> resource/quantitative_results_gen.tex <==
\begin{table}[t]
\caption{Unconditional video generation. UCF-101 with 128 frames... FVDs...
}\label{tab:long-video-generation} 
\centering\small
\vspace{-0.15in}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lc}
\toprule
Method & FVD$\downarrow$ \\
\midrule
MoCoGAN \citep{tulyakov2018mocogan} & 3679.0 \\
+ StyleGAN2 \citep{karras2020analyzing} & 2311.3 \\
MoCoGAN-HD \citep{tian2021good} & 2606.5 \\
DIGAN \citep{yu2022generating} & 2293.7 \\
StyleGAN-V \citep{skorokhodov2022stylegan} & 1773.4 \\
PVDM-L \citep{yu2023video} & \phantom{0}505.0 \\
HVDM \citep{kim2024hybrid} & \phantom{0}549.7 \\
\midrule
\sname-SiT-L/2 (Ours) & \phantom{0}\bf{369.3} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\begin{table}[t]
\caption{Inference efficiency of video generation models for synthesizing a 128 frame length and $128\times128$ resolution video. We use a DDIM sampler for PVDM and HVDM, and a Heun sampler for Ours. We measure all the results with a single NVIDIA 4090 24GB GPU.}
% \huiwon{Will change to the graph (training efficiency / inference efficiency) ASAP: Effect of efficient tokenization for train / inference efficiency of generative models..}}
\label{tab:long-video-generation-efficiency} 
\centering\small
\vspace{-0.05in}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lccc}
\toprule
Method  & Sampling steps & time (s) & memory (GB) \\
\midrule
TATS & - & \\
LARP & - & \\
\midrule
PVDM-L \citep{yu2023video} & 200 & $> 64$ & 4.03 \\
HVDM \citep{kim2024hybrid} & & \\
\midrule
\sname-SiT-L/2 (Ours) & 250 & \textbf{9.84} & 4.49 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

